User Review-Based Change File Localization for Mobile Applications

In the current mobile app development, novel and emerging DevOps practices (e.g., Continuous Delivery, Integration, and user feedback analysis) and tools are becoming more widespread. For instance, the integration of user feedback (provided in the form of user reviews) in the software release cycle represents a valuable asset for the maintenance and evolution of mobile apps. To fully make use of these assets, it is highly desirable for developers to establish semantic links between the user reviews and the software artefacts to be changed (e.g., source code and documentation), and thus to localize the potential files to change for addressing the user feedback. In this paper, we propose RISING (Review Integration via claSsification, clusterIng, and linkiNG), an automated approach to support the continuous integration of user feedback via classification, clustering, and linking of user reviews. RISING leverages domain-specific constraint information and semi-supervised learning to group user reviews into multiple fine-grained clusters concerning similar users' requests. Then, by combining the textual information from both commit messages and source code, it automatically localizes potential change files to accommodate the users' requests. Our empirical studies demonstrate that the proposed approach outperforms the state-of-the-art baseline work in terms of clustering and localization accuracy, and thus produces more reliable results.

==> sections/embedding.tex <==

\section{A brief survey of word embedding and related techniques}

Everything starts from the \emph{distributional hypothesis} (Harris 1954): a feature is characterized by the words in its context". 

Low-dimensional vector embeddings are a popular approach for capturing the ``meaning" of text and a form of unsupervised learning useful for downstream tasks. 

We focus on linear embedding schemes. 

\subsection{Word embedding}

Distributional word embeddings, which represent the ``meaning" of a word via a low-dimensional vector, have been widely applied by many NLP pipelines and algorithms. 

There are two representative work. 

\begin{itemize}
	\item Neural approach (Mikolov NIPS'13)
	
	\item matrix factorization method (Pennington, Glove, EMNLP)
	
\end{itemize}


Word2vec is a group of related models that are used to produce word embeddings. These models are shallow, two-layer neural networks that are trained to reconstruct linguistic contexts of words. Word2vec takes as its input a large corpus of text and produces a vector space, typically of several hundred dimensions, with each unique word in the corpus being assigned a corresponding vector in the space. Word vectors are positioned in the vector space such that words that share common contexts in the corpus are located in close proximity to one another in the space.

Word2vec was created by a team of researchers led by Tomas Mikolov at Google. The algorithm has been subsequently analysed and explained by other researchers. Embedding vectors created using the Word2vec algorithm have many advantages compared to earlier algorithms  such as latent semantic analysis.


Software

Software for training and using word embeddings includes Tomas Mikolov's Word2vec, Stanford University's GloVe,[21] AllenNLP's Elmo,[22] fastText, Gensim,[23] Indra[24] and Deeplearning4j. Principal Component Analysis (PCA) and T-Distributed Stochastic Neighbour Embedding (t-SNE) are both used to reduce the dimensionality of word vector spaces and visualize word embeddings and clusters.[25]



\textbf{CBOW and skip grams}

Word2vec can utilize either of two model architectures to produce a distributed representation of words: continuous bag-of-words (CBOW) or continuous skip-gram. In the continuous bag-of-words architecture, the model predicts the current word from a window of surrounding context words. The order of context words does not influence prediction (bag-of-words assumption). In the continuous skip-gram architecture, the model uses the current word to predict the surrounding window of context words. The skip-gram architecture weighs nearby context words more heavily than more distant context words.  According to the authors' note, CBOW is faster while skip-gram is slower but does a better job for infrequent words.

%http://mccormickml.com/2016/04/19/word2vec-tutorial-the-skip-gram-model/

\paragraph{Basic principle of word2vec}

unsupervised Skip-gram model which learns vector representation of words that are useful for predictiing the surrounding words in a sentence. 

The vector representation of $w_t$ is used as the parameter vector of  a binary logistic regression model $P[w_k\in C_t\mid w_t]$

%=====================================================================================
%======================================================================================
\subsection{Extensions}

Word embeddings computed using diverse methods are basic building blocks for Natural Language
Processing (NLP) and Information Retrieval (IR).  

Following the success of word embedding, researchers seek to \textbf{extend to other text features, from subword elements to n-grams to sentences}. 

Issues: the performance of both word embeddings and their extensions is known to degrade \textbf{in small corpus settings} or when embedding sparse, low-frequency features. 

For computational efficiency it is desirable that methods be able to induce embeddings for only those features (e.g. bigrams or synsets) needed by the downstream task, rather than having to pay a computational prix fiex to learn embeddings for all features occurring frequently-enough in a corpus. 

\paragraph{a la carte embedding} a method which bootstraps existing high-quality word vectors to learn a feature representation in the same semantic space via a linear transformation of the average word embeddings in the features's availabel contexts. 


Assume a large text corpus $C_V$ consisting of contexts $c$ of words $w$ in a vocabulary $V$ with contexts themselves being sequences of words in $V$ (e.g. a fixed-size window around the word or feature). We further assume that we have trained word embedding s $v_w\in R^d$ on this collocation information using a standard algorithm (e.g. word2vec and GloVe). The goal is to construct a good embedding $v_f\in R^d$ of a text feature $f$ given a set $C_f$ of contexts it occurs in. (Both $f$ and its contexts are assumed to arise via the same process that generates the large corpus $C_V$.) In many settings, the number $|C_f|$ of contexts available for a feature $f$ of interests is much smaller than the number $|C_w|$ of contexts that the typical word $w\in V$ occurs in. This could be becasue the feature is rare or due to limited human annotations. 

Additive Approach: take the average over all contexts of a feature $f$ of the average word vector in each context
\[v_f:=\frac{1}{|C_f|} \sum_{c\in C_f} \frac{1}{|c|}\sum_{w\in c} v_w \]
	
A natural extension is to use an arbitaray linear transformation which will be learned from the data,a nd hence guaranteed to do at least as well as ...

This can be posed as the following linear regression problem 
\[v_w\approx Av_w^a = A\left(\frac{1}{|C_f|} \sum_{c\in C_w}\sum_{w'\in c}  v_{w'}\right)\]	

After learning the matrix $A$, we can embed any text feature in the same semantics space as the word embeddings via the following expression. 
	

\subsection{A SIMPLE BUT TOUGH-TO-BEAT BASELINE FOR SENTENCE EMBEDDINGS}


\paragraph{Phrase/Sentence/Paragraph embeddings.}

Previous works have computed phrase or sentence
embeddings by 

\begin{itemize}
	\item composing word embeddings using operations on vectors and matrices e.g.,
	(Mitchell \& Lapata, 2008; 2010; Blacoe \& Lapata, 2012). They found that coordinate-wise multiplication 	of the vectors performed very well among the binary operations studied. Unweighted averaging 	is also found to do well in representing short phrases (Mikolov et al., 2013a). 
	
	\item Another approach 	is recursive neural networks (RNNs) defined on the parse tree, trained with supervision (Socher et al., 2011) or without (Socher et al., 2014). Simple RNNs can be viewed as a special case where the parse tree is replaced by a simple linear chain. For example, the skip-gram model (Mikolov et al., 2013b) is extended to incorporate a latent vector for the sequence, or to treat the sequences rather than the word as basic units. In (Le \& Mikolov, 2014) each paragraph was assumed to have a latent paragraph vector, which influences the distribution of the words in the paragraph. Skip-thought of (Kiros et al., 2015) tries to reconstruct the surrounding sentences from surrounded one and treats
	the hidden parameters as their vector representations. 
	
	RNNs using long short-term memory (LSTM) capture long-distance dependency and have also been used for modeling sentences (Tai et al., 2015).	Other neural network structures include convolution neural networks, such as (Blunsom et al., 2014)	that uses a dynamic pooling to handle input sentences of varying length and do well in sentiment
	prediction and classification tasks.
	
\end{itemize}


%\paragraph{LSTM representation}
%
%The success of neural network methods for computing word embeddings has motivated
%methods for generating semantic embeddings of longer pieces of text, such
%as sentences and paragraphs.
%
%LSTMs have become a common way to apply the expressive power of RNNs, with success on a variety of classification, representation and sequence-to-sequence tasks. For document representation, ...
%

%
%\begin{itemize} 
%\item Based on the latent variable generative model fro text. 
%
%\item CBOW model of word2vec
%\end{itemize}

The sentence embedding algorithm:

Input: word embeddings $\{v_w\mid w\in V\}$, a set of sentences $S$, parameter $a$ and estimated probabilities $\{p(w) \mid w\in V\}$ of words. Output: sentence embedding $\{v_s\mid s\in S\}$. 

\[v_s:= \frac{1}{|s|}\sum_{w\in s} \frac{a}{a+p(w)} v_w\]
		
Form a matrix $X$ whose columns are $\{v_s\mid s\in S\}$, and let $u$ be its first singular vector, and then ...

The authors compare their method with the following

\begin{itemize} 
\item Unsupervised: ST, avg-GloVe, tfidf-GloVe. ST denotes the skip-thought vectors (Kiros
 et al., 2015), avg-GloVe denotes the unweighted average of the GloVe vectors (Pennington
 et al., 2014) and tfidf-GloVe denotes the weighted average of GloVe vectors using TF-IDF weights.
 
 [In information retrieval, tf–idf or TFIDF, short for term frequency–inverse document frequency, is a numerical statistic that is intended to reflect how important a word is to a document in a collection or corpus. It is often used as a weighting factor in searches of information retrieval, text mining, and user modeling. The tf–idf value increases proportionally to the number of times a word appears in the document and is offset by the number of documents in the corpus that contain the word, which helps to adjust for the fact that some words appear more frequently in general.]

 
\item Semi-supervised: avg-PSL. This method uses the unweighted average of the PARAGRAMSL999
 (PSL) word vectors from (Wieting et al., 2015). The word vectors are trained using
 labeled data, but the sentence embedding are computed by unweighted average without
 training.

\item Supervised: PP, PP-proj., DAN, RNN, iRNN, LSTM (o.g.), LSTM (no). All these methods
 are initialized with PSL word vectors and then trained on the PPDB dataset. PP and PPproj.
 are proposed in (Wieting et al., 2016). The first is an average of the word vectors, and
 the second additionally adds a linear projection. The word vectors are updated during the
 training. DAN denotes the deep averaging network of (Iyyer et al., 2015). RNN denotes the
 classical recurrent neural network, and iRNN denotes a variant with the activation being the
 identity, and the weight matrices initialized to identity. The LSTM is the version from (Gers
 et al., 2002), either with output gates (denoted as LSTM(o.g.)) or without (denoted as
 LSTM (no)).

\end{itemize}

\subsection{A framework of text embedding}

Let $V$ be the number of words in the vocabulary and $V_n$ be the number of $n$-grams (independent of word order), so that $V=V_1$. 

\textbf{Bag-of-n-grams vector} Assigning to each word a unique index $i\in [V]$ we define the BoW representation of a document to be the V-dimensional vector whose $i$-th entry is the number times word $i$ occurs in the document. 

The n-gram extension is the Bag-of-n-grams (BonG) representation, which counts the number of times any $k$-gram for $k\leq n$ appears in a document. 

\begin{itemize}
	\item unigram embedding
	\item 
\end{itemize}

Useful references:

John Wieting, Mohit Bansal, Kevin Gimpel, and Karen Livescu. Towards universal paraphrastic
sentence embeddings. In International Conference on Learning Representations, 2016.

%===================================================================
% doc2vec
%===================================================================

\section{document2word}

%https://radimrehurek.com/gensim/models/doc2vec.html

The algorithms use either hierarchical softmax or negative sampling; see Tomas Mikolov, Kai Chen, Greg Corrado, and Jeffrey Dean: “Efficient Estimation of Word Representations in Vector Space, in Proceedings of Workshop at ICLR, 2013” and Tomas Mikolov, Ilya Sutskever, Kai Chen, Greg Corrado, and Jeffrey Dean: “Distributed Representations of Words and Phrases and their Compositionality. In Proceedings of NIPS, 2013”.

For a usage example, see the Doc2vec tutorial.

https://github.com/RaRe-Technologies/gensim/blob/develop/docs/notebooks/doc2vec-lee.ipynb

Make sure you have a C compiler before installing Gensim, to use the optimized doc2vec routines (70x speedup compared to plain NumPy implementation, https://rare-technologies.com/parallelizing-word2vec-in-python/).

https://rare-technologies.com/parallelizing-word2vec-in-python/

A gentle introduction to Doc2Vec: 

https://medium.com/scaleabout/a-gentle-introduction-to-doc2vec-db3e8c0cce5e

%Distributed Representations of Sentences and Documents
%Quoc Le, Tomas Mikolov ICML'14


currently: Many machine learning algorithms require the
input to be represented as a \textbf{fixed-length feature
	vector}. When it comes to texts, one of the most
common fixed-length features is bag-of-words.
Despite their popularity, \textbf{bag-of-words features}
have two major weaknesses: they lose the ordering
of the words and they also ignore semantics
of the words. 



For example, “powerful,” “strong”
and “Paris” are equally distant. 

Now: \emph{Paragraph Vector}, an unsupervised algorithm
that learns \textbf{fixed-length feature representations}
from variable-length pieces of texts, such as
sentences, paragraphs, and documents. Our algorithm
represents each document by a dense vector
which is trained to predict words in the document.

%Its construction gives our algorithm the
%potential to overcome the weaknesses of bag-of-words
%models. Empirical results show that Paragraph
%Vectors outperform bag-of-words models
%as well as other techniques for text representations.
%Finally, we achieve new state-of-the-art results
%on several text classification and sentiment
%analysis tasks.

Even though bag-of-n-grams considers
the word order in short context, it suffers from data
sparsity and high dimensionality.

Bag-of-words and bag-of-n-grams
have very little sense about the semantics of the
words or more formally the distances between the words.
This means that words “powerful,” “strong” and “Paris” are
equally distant despite the fact that semantically, “powerful”
should be closer to “strong” than “Paris.”

\cite{LM14} proposed Paragraph Vector, an unsupervised
framework that learns continuous distributed vector
representations for pieces of texts. The texts can be of
variable-length, ranging from sentences to documents. The
name Paragraph Vector is to emphasize the fact that the
method can be applied to variable-length pieces of texts,
anything from a phrase or sentence to a large document.


Following these successful techniques, researchers have
tried to extend the models to go beyond word level
to achieve phrase-level or sentence-level representations
(Mitchell \& Lapata, 2010; Zanzotto et al., 2010;
Yessenalina \& Cardie, 2011; Grefenstette et al., 2013;
Mikolov et al., 2013c).  


A particular implementation of neural network based algorithm
for training the word vectors is available at code.google.com/p/word2vec/ (Mikolov et al.,
2013a).


\begin{itemize}
	\item  Paragraph Vector: A distributed memory model
	\item  Paragraph Vector without word ordering:
	Distributed bag of words
\end{itemize}

%==========================================================================
\section{Topic model}

%The following material is from the paper learning topic models going beyond SVD

In order to learn structure one has to posit the existence of a structure. In topic models, one assumes that a generative model for a collection of documents. Specially, each document is represented as a vector of word frequencies (the bag of words representation). 

The documents areise as a convex combination of (i.e. distributon on) a small number of topic vectors, where each topic vector is a distribution on words (i.e., a vector of word-frequencies). 

Subsequent work makes specific choices for the distribution used to generate topic combinations. (the well known LDA model of Blei hypothesizes a Dirichlet distribution. )

\section{NMF meets word embedding}

Setting: document clustering; traditional approach NMF but they use the bag-of-words representation and thus  do not account for the sequential order in which words occur in documents. 

word embedding: proven effiective in learning continuous representations of words that successfully capture meaningful syntactic and semantic regularities between words. Given a corpus of unannotated text documents, each of which represented as a sequence of words, the contexts for word $w$ are the words surrounding it in an L-sized window in any document of the corpus. We assume that frequently co-occurring words in an L-size window in any document are likely to have a common meaning. 

Method: Semantics-NMF which jointly decomposes the document-word and word-context co-occurrence matrices with shared word factors. The decomposition of the word-context matrix has been shown to be equivalent to a state of the art neural word embedding method, namely the skip-gram model. 

==> sections/semisupervised.tex <==

 
\section{Semi-supervised clustering methods}

We will now briefly outline several semi-supervised clustering methods. These methods
will be organized according to the nature of the known outcome data. 

\subsection{the data is partially labeled} 

Basu et al. developed a generalization of k-means clustering (which they called “constrained
k-means”) for the situation where class labels are known for a subset of the
observations.

\subsection{Relationship between the features is known}

Clustering when more complex relationships among the observations
are known. In particular, 
two types of possible constraints among
observations: 

``Must-link constraints" require that two observations must be placed in
the same cluster, and ``cannot-link constraints" require that two observations must not
be placed in the same cluster. 

Numerous methods have been proposed for solving the problem of constrained clustering.
[Survey book] Basu S, Davidson I, Wagstaff K. Constrained Clustering: Advances in Algorithms,
Theory, and Applications. Chapman Hall/CRC Data Mining and
Knowledge Discovery Series. CRC Press, Boca Raton, FL, 2009.

The methods  modify an existing clustering method (namely k-means
clustering) such that the constraints are satisfied. Thus, such methods are sometimes
referred to as “constraint-based methods” in literature. In contrast, “distance based
methods” (or “metric-based methods”) use an existing clustering method but
modify the metric used to measure the “distance” between a pair of observations such
that the constraints are satisfied. 

[For example, rather than using the simple Euclidean
distance, one may use an alternative distance metric such that two observations
with a “must-link constraint” will necessarily have a lower distance between them.]

Moreover, other constraint-based methods have been proposed, and still other
methods combine both of these approaches into a single model. Other forms of
constrained clustering are also possible, such as clustering on graph data.  

\subsection{identify clusters associated with a particular
outcome variable}

